Monitoring multidimensional phenomena with a multicriteria composite performance interval approach

In the last two decades, composite indicators' construction to measure and compare multidimensional phenomena in a broad spectrum of domains has increased considerably. Different methodological approaches are used to summarize huge data sets of information in a single figure. This paper proposes a new approach that consists of computing a multicriteria composite performance interval based on different aggregation rules. The suggested approach provides an additional layer of information as the performance interval displays a lower bound from a non-compensability perspective, and an upper bound allowing for full-compensability. The outstanding features of this proposal are: (i) a distance-based multicriteria technique is taken as the baseline to construct the multicriteria performance interval (ii) the aggregation of distances/separation measures is made using particular cases of Minkowski's $L_p$ metrics; (iii) the span of the multicriteria performance interval can be considered as a sign of the dimensions or indicators balance.

==> table_MCPI_by_dim_Europe_but_CI.tex <==
\begin{tabular}{ l r@{\hspace{2pt}}  r@{\hspace{4pt}}  r  r@{\hspace{2pt}}  r@{\hspace{4pt}}  r  r@{\hspace{2pt}}  r@{\hspace{4pt}}  r}

\toprule

 &  \multicolumn{3}{c}{$\delta_\mathrm{PC}$} & \multicolumn{3}{c}{$\delta_\mathrm{WM}$} & \multicolumn{3}{c}{$\delta_\mathrm{SRM}$} \\

\midrule

Austria	&	[	&	43.4,	&	83.2\hspace{2pt}]	&	[	&	80.0,	&	81.8\hspace{2pt}]	&	[	&	23.4,	&	29.5\hspace{2pt}]	&	[	&	8.1,	&	30.7\hspace{2pt}] \\
Belgium	&	[	&	4.7,	&	63.4\hspace{2pt}]	&	[	&	77.8,	&	87.3\hspace{2pt}]	&	[	&	72.6,	&	73.8\hspace{2pt}]	&	[	&	0.0,	&	37.5\hspace{2pt}] \\
Bulgaria	&	[	&	23.0,	&	44.2\hspace{2pt}]	&	[	&	24.3,	&	31.1\hspace{2pt}]	&	[	&	3.5,	&	4.1\hspace{2pt}]	&	[	&	0.0,	&	24.6\hspace{2pt}] \\
Croatia	&	[	&	70.5,	&	86.3\hspace{2pt}]	&	[	&	26.8,	&	43.1\hspace{2pt}]	&	[	&	3.0,	&	7.5\hspace{2pt}]	&	[	&	15.5,	&	40.5\hspace{2pt}] \\
Cyprus*	&	[	&	32.7,	&	87.7\hspace{2pt}]	&	[	&	10.7,	&	20.2\hspace{2pt}]	&	[	&	0.0,	&	2.1\hspace{2pt}]	&	[	&	0.0,	&	22.8\hspace{2pt}] \\
Czechia	&	[	&	77.5,	&	90.2\hspace{2pt}]	&	[	&	42.9,	&	56.9\hspace{2pt}]	&	[	&	6.2,	&	14.7\hspace{2pt}]	&	[	&	9.3,	&	37.1\hspace{2pt}] \\
Denmark	&	[	&	0.0,	&	80.0\hspace{2pt}]	&	[	&	69.9,	&	71.3\hspace{2pt}]	&	[	&	9.6,	&	16.7\hspace{2pt}]	&	[	&	7.1,	&	35.6\hspace{2pt}] \\
Estonia	&	[	&	0.0,	&	12.2\hspace{2pt}]	&	[	&	0.0,	&	16.1\hspace{2pt}]	&	[	&	4.0,	&	23.7\hspace{2pt}]	&	[	&	28.3,	&	61.8\hspace{2pt}] \\
Finland	&	[	&	48.5,	&	85.0\hspace{2pt}]	&	[	&	38.6,	&	47.7\hspace{2pt}]	&	[	&	2.3,	&	8.9\hspace{2pt}]	&	[	&	24.7,	&	61.7\hspace{2pt}] \\
France	&	[	&	48.6,	&	81.6\hspace{2pt}]	&	[	&	61.1,	&	62.1\hspace{2pt}]	&	[	&	36.6,	&	50.8\hspace{2pt}]	&	[	&	10.8,	&	31.4\hspace{2pt}] \\
Germany	&	[	&	38.4,	&	79.5\hspace{2pt}]	&	[	&	61.4,	&	81.1\hspace{2pt}]	&	[	&	38.2,	&	70.1\hspace{2pt}]	&	[	&	9.2,	&	36.7\hspace{2pt}] \\
Greece	&	[	&	49.5,	&	78.3\hspace{2pt}]	&	[	&	17.7,	&	23.7\hspace{2pt}]	&	[	&	6.4,	&	8.4\hspace{2pt}]	&	[	&	0.0,	&	6.8\hspace{2pt}] \\
Hungary	&	[	&	70.3,	&	88.9\hspace{2pt}]	&	[	&	46.6,	&	47.6\hspace{2pt}]	&	[	&	5.1,	&	12.3\hspace{2pt}]	&	[	&	13.9,	&	30.0\hspace{2pt}] \\
Ireland	&	[	&	39.9,	&	88.1\hspace{2pt}]	&	[	&	44.3,	&	46.4\hspace{2pt}]	&	[	&	0.3,	&	1.7\hspace{2pt}]	&	[	&	9.3,	&	30.9\hspace{2pt}] \\
Italy	&	[	&	30.0,	&	70.3\hspace{2pt}]	&	[	&	69.7,	&	76.2\hspace{2pt}]	&	[	&	61.9,	&	63.2\hspace{2pt}]	&	[	&	8.9,	&	30.7\hspace{2pt}] \\
Latvia	&	[	&	75.1,	&	93.1\hspace{2pt}]	&	[	&	0.0,	&	13.6\hspace{2pt}]	&	[	&	4.3,	&	8.1\hspace{2pt}]	&	[	&	19.8,	&	46.1\hspace{2pt}] \\
Lithuania	&	[	&	59.5,	&	83.8\hspace{2pt}]	&	[	&	74.4,	&	78.6\hspace{2pt}]	&	[	&	7.8,	&	8.9\hspace{2pt}]	&	[	&	0.0,	&	34.0\hspace{2pt}] \\
Luxembourg	&	[	&	2.0,	&	78.6\hspace{2pt}]	&	[	&	68.3,	&	72.6\hspace{2pt}]	&	[	&	17.7,	&	25.5\hspace{2pt}]	&	[	&	100.0,	&	100.0\hspace{2pt}] \\
Malta	&	[	&	27.9,	&	82.6\hspace{2pt}]	&	[	&	0.0,	&	23.1\hspace{2pt}]	&	[	&	0.8,	&	12.0\hspace{2pt}]	&	[	&	0.0,	&	0.0\hspace{2pt}] \\
Netherlands	&	[	&	10.1,	&	65.1\hspace{2pt}]	&	[	&	80.4,	&	84.4\hspace{2pt}]	&	[	&	88.1,	&	93.9\hspace{2pt}]	&	[	&	2.4,	&	32.9\hspace{2pt}] \\
Poland	&	[	&	53.7,	&	79.4\hspace{2pt}]	&	[	&	41.7,	&	53.5\hspace{2pt}]	&	[	&	17.2,	&	23.3\hspace{2pt}]	&	[	&	26.6,	&	56.0\hspace{2pt}] \\
Portugal	&	[	&	56.6,	&	85.8\hspace{2pt}]	&	[	&	33.5,	&	46.5\hspace{2pt}]	&	[	&	2.2,	&	8.5\hspace{2pt}]	&	[	&	0.0,	&	17.0\hspace{2pt}] \\
Romania	&	[	&	64.0,	&	90.9\hspace{2pt}]	&	[	&	1.9,	&	15.0\hspace{2pt}]	&	[	&	0.0,	&	4.0\hspace{2pt}]	&	[	&	5.8,	&	17.3\hspace{2pt}] \\
Slovakia	&	[	&	62.1,	&	81.6\hspace{2pt}]	&	[	&	46.1,	&	47.3\hspace{2pt}]	&	[	&	3.5,	&	8.0\hspace{2pt}]	&	[	&	0.8,	&	16.8\hspace{2pt}] \\
Slovenia	&	[	&	60.5,	&	83.6\hspace{2pt}]	&	[	&	85.6,	&	92.7\hspace{2pt}]	&	[	&	7.9,	&	19.1\hspace{2pt}]	&	[	&	0.0,	&	29.9\hspace{2pt}] \\
Spain	&	[	&	42.6,	&	76.9\hspace{2pt}]	&	[	&	43.4,	&	47.4\hspace{2pt}]	&	[	&	29.4,	&	40.1\hspace{2pt}]	&	[	&	18.1,	&	39.8\hspace{2pt}] \\
Sweden	&	[	&	70.1,	&	89.1\hspace{2pt}]	&	[	&	55.7,	&	59.3\hspace{2pt}]	&	[	&	16.2,	&	17.5\hspace{2pt}]	&	[	&	9.6,	&	28.0\hspace{2pt}] \\
United Kingdom	&	[	&	31.1,	&	72.7\hspace{2pt}]	&	[	&	59.7,	&	64.1\hspace{2pt}]	&	[	&	53.8,	&	73.5\hspace{2pt}]	&	[	&	8.6,	&	29.9\hspace{2pt}] \\

\bottomrule

\end{tabular}

